Abundance stratification in Type Ia supernovae - V. SN 1986G bridging the gap between normal and subluminous SNe Ia

A detailed spectroscopic analysis of SN 1986G has been performed. SN 1986G `bridges the gap' between normal and sub luminous type Ia supernova (SNe Ia). The abundance tomography technique is used to determine the abundance distribution of the elements in the ejecta. SN 1986G was found to be a low energy Chandrasekhar mass explosion. Its kinetic energy was 70% of the standard W7 model (0.9x10$^{51}$erg). Oxygen dominates the ejecta from the outermost layers down to $\sim$9000kms$^{-1}$ , intermediate mass elements (IME) dominate from $\sim$ 9000kms$^{-1}$ to $\sim$ 3500kms$^{-1}$ with Ni and Fe dominating the inner layers $<\sim$ 3500kms$^{-1}$. The final masses of the main elements in the ejecta were found to be, O=0.33M, IME=0.69M, stable NSE=0.21M, $^{56}$Ni=0.14M. An upper limit of the carbon mass is set at C=0.02M. The spectra of SN1986G consist of almost exclusively singly ionised species. SN1986G can be thought of as a low luminosity extension of the main population of SN Ia, with a large deflagration phase that produced more IMEs than a standard SN Ia.

==> README <==
% readme.txt
%
% MNRAS journal LaTeX package
% v3.0 for LaTeX 2e
%
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `author-maintained'.
% 
% The Current Maintainer of this work is: Royal Astronomical Society,
% MNRAS Editorial Office, who can be contacted on mn@ras.org.uk
%
% This work consists of all the files listed in readme.txt
%
%
% Last updated 22 May 2015
%
% Copyright (C) Royal Astronomical Society 2015, Blackwell Science 2001,
% Cambridge University Press 1994
%
% See each file for a detailed author list and change log.
%
% This package consists of the following files:

readme.txt          This file

mnras.cls           MNRAS LaTeX document class
mnras.bst           MNRAS BibTeX style

mnras_guide.tex     User guide, LaTeX format
mnras_guide.pdf     User guide, PDF format
mnras_template.tex  A simple template paper

example.eps         An example image used in the guide
example.png         An example image used in the guide
example.ps          An example image used in the guide

legacy\legacy.txt   Description of the legacy releases
legacy\mn2e.cls     v2.2 of mn2e.cls (deprecated)
legacy\mn2e.bst     v1.1b of mn2e.bst (deprecated)


% Disclaimer:
%
% This LaTeX package is provided free to the community in the hope that it
% assists them in preparing papers for the journal Monthly Notices of the
% Royal Astronomical Society.
% The files are provided 'as-is' with no guarantee of their suitability,
% freedom from errors or omissions, or compatibility with any software.
% The Royal Astronomical Society cannot provide user support for this package,
% LaTeX, or for any other software.
% Authors are free to use other styles or programmes if they wish.
% Please see the journal instructions to authors for guidance.
% This disclaimer is in addition to the No Warranty section of the licence,
% at the link given above.
